Flow Map Learning for Unknown Dynamical Systems: Overview, Implementation, and Benchmarks

Flow map learning (FML), in conjunction with deep neural networks (DNNs), has shown promises for data driven modeling of unknown dynamical systems. A remarkable feature of FML is that it is capable of producing accurate predictive models for partially observed systems, even when their exact mathematical models do not exist. In this paper, we present an overview of the FML framework, along with the important computational details for its successful implementation. We also present a set of well defined benchmark problems for learning unknown dynamical systems. All the numerical details of these problems are presented, along with their FML results, to ensure that the problems are accessible for cross-examination and the results are reproducible.

==> Conclusion.tex <==
\section{Conclusion} \label{sec:conclusions}

We presented a deep learning strategy for modeling unknown dynamical
systems with hidden parameters. By incorporating both memory terms in
the network input layer and
recurrent terms in the network loss function computation, the proposed
DNN is able to learn the unknown flow map of the system, by only using
trajectory data of the state variables. A distinct feature of the DNN
structure is that it is able to model the system with completely
hidden and unknown parameters. This can be useful for practical
problems, where many system parameters can not be measured. The
proposed DNN method thus provides a highly flexible approach for learning
unknown dynamical systems.
